The Optimal Pebbling Number of Staircase Graphs

Let G be a graph with a distribution of pebbles on its vertices. A pebbling move consists of removing two pebbles from one vertex and placing one pebble on an adjacent vertex. The optimal pebbling number of G is the smallest number of pebbles which can placed on the vertices of G such that, for any vertex v of G, there is a sequence of pebbling moves resulting in at least one pebble on v. We determine the optimal pebbling number for several classes of induced subgraphs of the square grid, which we call staircase graphs.

==> tikzstyles.tex <==

\tikzset{pebble/.style={shape          = circle,
                                 ball color     = blue,
                                 text           = white,
                                 inner sep      = 2pt,
                                 outer sep      = 0pt,}};
\tikzset{pebble2/.style={shape          = circle,
                                 ball color     = violet!50,
                                 text           = red,
                                 inner sep      = 2pt,
                                 outer sep      = 0pt,}};
\tikzset{tipus/.style={shape          = rectangle,
                                % ball color     = violet!10,
                                fill = white,
                                 text           = black,
                                 inner sep      = 0pt,
                                 outer sep      = 0pt,}};
\tikzset{csucs/.style={ circle,
                                % ball color     = violet!10,
                                fill = white,
                                % text           = black,
                                 inner sep      = 0pt,
                                 outer sep      = 0pt,
																}};
 \tikzset{szaggatott/.style={ultra thick, dashed}};
\tikzstyle{every path} = [>=stealth];
\tikzset{koord/.style={draw}};
\tikzstyle{nyil} = [>=latex,very thick,->];
